Factorization-free Orthogonal Projection onto the Positive Semidefinite Cone with Composite Polynomial Filtering

We propose a factorization-free method for orthogonal projection onto the positive semidefinite (PSD) cone, leveraging composite polynomial filtering. Inspired by recent advances in homomorphic encryption, our approach approximates the PSD cone projection operator using a carefully optimized composite polynomial evaluated exclusively via matrix-matrix multiplications. This approach enables efficient GPU implementations with low-precision arithmetic, significantly outperforming the classical PSD cone projection using state-of-the-art GPU-based eigenvalue decomposition solvers. Specifically, our method achieves a consistent relative error of $10^{-3}$ in half-precision arithmetic with only 22 matrix-matrix multiplications, providing roughly a $10\times$ speed-up over NVIDIA's cuSOLVER routines on various large-scale matrices. In single-precision arithmetic with emulation on B200 GPUs, our approach maintains competitive accuracy while achieving up to a $2\times$ speed-up. Consequently, for a $10,000 \times 10,000$ dense symmetric matrix, our method requires approximately $55$ ms in half-precision and $400$ ms in single-precision arithmetic on B200 GPUs. Integration into a first-order semidefinite programming solver confirms that our low-precision projections reliably yield solutions of moderate accuracy.

==> figs/comparison.tex <==
%!TEX root = ../main.tex

\begin{figure}[tbp]
    \centering

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/f_1.png}
                Newton-Schulz iteration
            \end{minipage}

            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/ours_2.png}
                Remez with sparse basis
            \end{minipage}

            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/ours.png}
                Remez + analytical formula
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{Approximation error with 30 multiplications. \label{fig:comparison}}
\end{figure}

==> references/preamble_packages.tex <==
%!TEX root = main.tex

\usepackage[utf8]{inputenc}
\usepackage{cite} % Optional: formats numeric citations nicely
\usepackage[vlined,ruled,linesnumbered]{algorithm2e}
\usepackage[noend]{algorithmic}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{prettyref}
\usepackage{xspace}
\usepackage{bm}
\usepackage{hyperref}
 


==> references/preamble_symbols.tex <==
%!TEX root = main.tex

% colors
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\cyan}[1]{{\color{cyan}#1}}
\newcommand{\gray}[1]{{\color{gray}#1}}

% manage references
\newcommand{\linkToPdf}[1]{\href{#1}{\blue{(pdf)}}}
\newcommand{\linkToCode}[1]{\href{#1}{\blue{(code)}}}
\newcommand{\linkToWeb}[1]{\href{#1}{\blue{(web)}}}
\newcommand{\linkToVideo}[1]{\href{#1}{\blue{(video)}}}
\newcommand{\linkToMedia}[1]{\href{#1}{\blue{(media)}}}
\newcommand{\award}[1]{\red{#1}}
% \newcommand{\award}[1]{\xspace} % omit awards


% common shortcuts
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\wrt}{w.r.t.\xspace}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beal}{\beq \begin{array}{ll}}
\newcommand{\eeal}{\end{array} \eeq}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\expl}[1]{&&\qquad\text{\color{gray}(#1)}\nonumber}

\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}\xspace}
\newcommand{\SE}[1]{\ensuremath{\mathrm{SE}(#1)}\xspace}
\newcommand{\SEthree}{\ensuremath{\mathrm{SE}(3)}\xspace}
\newcommand{\SOtwo}{\ensuremath{\mathrm{SO}(2)}\xspace}
\newcommand{\SOthree}{\ensuremath{\mathrm{SO}(3)}\xspace}
\newcommand{\Othree}{\ensuremath{\mathrm{O}(3)}\xspace}
\newcommand{\SOn}{\ensuremath{\mathrm{SO}(n)}\xspace}
\newcommand{\SO}[1]{\ensuremath{\mathrm{SO}(#1)}\xspace}
\newcommand{\On}{\ensuremath{\mathrm{O}(n)}\xspace}
\newcommand{\sotwo}{\ensuremath{\mathrm{so}(2)}\xspace}
\newcommand{\sothree}{\ensuremath{\mathrm{so}(3)}\xspace}






==> sections/introduction.tex <==
%!TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

Consider the space of $n \times n$ symmetric matrices $\Sn$. Define the positive semidefinite (PSD) cone as $\psd{n} := \left\{ A \in \Sn \mymid A \succeq 0 \right\}$. 
Given a symmetric matrix $X$, the goal of PSD cone projection is to find the closest point in the PSD cone to $X$ with respect to the Frobenius norm:
\begin{align}
    \label{eq:intro:psdcone-proj}
    \PiSnp{X} := \argmin_{Y \in \psd{n}} \frac{1}{2} \norm{Y - X}_F^2
\end{align}
In both linear and nonlinear semidefinite programming (SDP), projection onto the PSD cone is arguably one of the most fundamental operators~\cite{wen2010mp-admmsdp,kang2025arxiv-local-linear-admmsdp}. There are two main-stream methods to compute PSD cone projection: (1) Direct computation via eigenvalue decomposition; (2) Iterative computation via polynomial/rational fixed point iteration.

\subsection{Direct computation via eigenvalue decomposition}
Since~\cite{higham1988laa-computing-psdcone-projection}, a widely accepted method for robust and accurate PSD cone projection is via eigenvalue decomposition:
\begin{align}
    \label{eq:intro:eig}
    X = V \Lambda V\tran, \quad \PiSnp{X} := V \max\left\{ \Lambda, 0 \right\} V\tran = V \begin{bmatrix}
        \max \left\{ \lambda_1, 0 \right\} & & \\
        & \ddots & \\
        & & \max \left\{ \lambda_n, 0 \right\}
    \end{bmatrix} V\tran 
\end{align}
where $V$ is an orthonormal matrix representing $X$'s eigenvectors and $\Lambda$ is a diagonal matrix representing $X$'s eigenvalues. A full eigenvalue decomposition of a general $n \times n$ symmetric matrix $X$ has a computational complexity of $\mathcal{O}(n^3)$ and a memory complexity of $\mathcal{O}(n^2)$, and is widely implemented across various computing architectures~\cite{anderson1999siam-lapack,lehoucq1998siam-arpack,cusolver,tomov2010pc-magma}. When either the positive or negative eigenvalue component is low-rank, PSD cone projection can be accelerated using low-rank eigenvalue decomposition algorithms~\cite{rontsis2022jota-approximate-admm}. Although sketching- and randomization-based methods for approximate large-scale PSD cone projection exist~\cite{jones2024arxiv-random-psdcone}, their convergence guarantees hold only in a probabilistic sense. All these methods explicitly relies on knowing (at least some) eigenvalue-eigenvector pairs. 

\subsection{Iterative computation via polynomial/rational fixed point iteration} 

Consider a spectral function generated by a scalar function $f(x): \mathbb{R} \mapsto \mathbb{R}$: 
\begin{align*}
    f(X) = V \begin{bmatrix}
        f(\lambda_1) & & \\
        & \ddots & \\
        & & f(\lambda_n)
    \end{bmatrix} V\tran, \quad \forall X = V \Lambda V\tran \in \Sn 
\end{align*}
From this perspective, PSD cone projection operator can be viewed as a spectral function generated by the scalar function $\max \left\{ x,0 \right\} = 0.5 x \cdot (1 + \sign(x))$~\cite{higham2008siam-functions-matrices,roberts1980ijc-linear-model}, where $\sign(x)$ is defined as:
\begin{align*}
    \sign(x) = \begin{cases}
        1, \ x > 0 \\
        0, \ x = 0 \\
        -1, \ x < 0
    \end{cases}
\end{align*}
The spectral function generated by $\sign(x)$ is called the matrix sign function~\cite{denman1976amc-matrix-sign}.

% \textit{Not every spectral function calculation needs eigen-pair information.} For instance, all matrix polynomial functions and matrix inversion (when $X$ is invertible) is eigenvalue-decomposition-free. These operators adopts better to large-scale parallel computation compared to full eigenvalue decomposition.
% Inspired by this, there has already been a rich body of literature using polynomial/rational fixed point iteration to calculate matrix sign function and polar factor, including Newton iteration~\cite{higham2008siam-functions-matrices,higham1986jssc-polar-decomposition}, inverse Newton iteration~\cite{nakatsukasa2010simaa-halley-polar}, and variants of Newton-Schulz iteration~\cite{chen2014anl-stable-newton-schulz,bjorc1971sina-iterative-estimate-orthogonal}. 
\textit{Not every computation of a matrix spectral function requires explicit eigen-pairs.}
Matrix polynomial functions and, when $X$ is invertible, the matrix inverse can both be evaluated without resorting to an eigenvalue decomposition.
These operators are usually more suited to large-scale parallel architectures, where the cost and communication overhead of full diagonalisation quickly become prohibitive.
Building on this observation, a substantial literature has developed polynomial- and rational-based fixed-point schemes for computing the matrix sign function and the polar factor.
Prominent examples include the Newton iteration~\cite{higham2008siam-functions-matrices,higham1986jssc-polar-decomposition}, the inverse Newton iteration~\cite{nakatsukasa2010simaa-halley-polar}, and several Newton--Schulz variants~\cite{chen2014anl-stable-newton-schulz,bjorc1971sina-iterative-estimate-orthogonal}.~\cite{amsel2025arxiv-polar-express} further utilizes a series of composition degree-5 minimax-optimal polynomials to calculate the matrix sign function to low accuracy and shows its great potential in deep learning training process.
Take the well-known inversion-free Newton-Schulz iteration as an example: 
\begin{align}
    \label{eq:intro:newton-schulz}
    X_{k+1} = g(X_k) := \frac{1}{2} X_k (3 I - X_k^2)  
\end{align}
Suppose all eigenvalue values of the starting point $X_0$ are within $[-1, 1]$. $\left\{ X_k \right\}_{k=1}^\infty$ will eventually converge to $\sign(X_0)$. One step further,~\cite{francisco2017laa-fixedpoint-approximate-psdcone} applies a variant of Newton--Schulz iteration to approximate sparse banded matrices' PSD cone projection. However, at the best of the author's knowledge, there is still no evidence showing that fixed-point-iteration-based PSD cone projection for dense matrix is truly competitive to eigenvalue-decomposition-based schemes in GPU. As previous works pointed out, fixed point iteration usually need too many iterations to converge to even median-accuracy solutions~\cite{chen2014anl-stable-newton-schulz,amsel2025arxiv-polar-express}. 

\subsection{Towards practical PSD cone projection with fixed-point iteration}

This work proposes a novel composite polynomial filtering scheme that enables fixed-point iterations to converge to single-precision accuracy within 30 matrix--matrix multiplications. Furthermore, we demonstrate that the Tensor Core-based computing architecture in GPU can significantly accelerate fixed-point projections onto the PSD cone, without compromising numerical accuracy.

\section{A New Composite Polynomial Filtering Scheme}

The approximation of the sign function has been extensively studied in the context of homomorphic comparison methods~\cite{cheon2020asiacrypt-efficient-homomorphic-comparison,lee2022tdsc-minimax-approximation-sign}. In~\cite{lee2022tdsc-minimax-approximation-sign}, the authors propose a routine for constructing a sequence of optimal composite functions based on minimax polynomial approximation. However, we observe that the notion of ``optimality'' in~\cite{lee2022tdsc-minimax-approximation-sign} is defined with respect to a fixed polynomial basis which span the space that contains all the polynomial whose degree is below a prescribed number $k_i$. In our setting, by contrast, the number of multiplications is the dominant constraint. For example, if we restrict the number of multiplications to $10$, the maximum achievable polynomial degree is $2^{10} = 1024$. However, these $10$ multiplications do not suffice to span the entire space of polynomials of degree at most $1024$.

\subsection{Sparse basis}

Since we would like to achieve median accuracy quickly, it is important for us to aggressively lift up the polynomial degrees within the limited number of multiplications. Inspired by Newton-Schulz iteration, we define our new ``basis'' as:
\begin{align}\label{eq:basis}
    x, \ \left\{ x \cdot (1 - x^2)^{2^k} \right\}_{k=0}^K \tag{BASIS}
\end{align}
To generate this set, we require only $K{+}1$ multiplications. This set can then be directly passed to the Remez algorithm to construct a feasible composite polynomial, as in~\cite{amsel2025arxiv-polar-express,lee2022tdsc-minimax-approximation-sign}. However, care must be taken, as our set of polynomials does not form a true basis for the space of polynomials of degree at most $2^K$. As a result, the Remez algorithm may fail to converge. Nevertheless, if the Remez algorithm does converge, the resulting coefficients are indeed minimax optimal over the given composite structure. In this case, we get our composite polynomial as 
\begin{align*}
    f_o(x) = c_{-1} \cdot x + \sum_{k=0}^K c_k \cdot x \cdot (1 - x^2)^{2^k}
\end{align*}
where ``o'' represents oscillating: $f_o$'s effect is to provide large slope near $0$. In the end of the composition, we also need some smoothing function to get high-accuracy approximation:
\begin{align*}
    f_s(x) = 1.5 x - 0.5 x^3
\end{align*}
which is exactly the Newton-Schulz iteration. 

\subsection{Problem statement}

Now we establish our scientific problem: 

\textit{Given a fixed number of multiplication, what is the best composite polynomial that minimize the approximation error of the ReLU function?}

We measure the approximation error in the $l_\infty$ norm using dense sampling. A natural idea is to approximate the ReLU function directly, but this creates difficulties when forming composite functions: because $\mathrm{ReLU}(x)$ has a non‐constant image, one cannot use a polynomial with a shrinking image to build the composite formula. Instead, we approximate the sign function and employ the identity: $\max \left\{ x,0 \right\} = 0.5 x \cdot (1 + \sign(x))$. 

To determine the composite polynomial $f_1 \circ f_2 \circ ... \circ f_n$, we must calculate \textbf{(i)} the degree (or degree of freedom here) of each $f_i$ and \textbf{(ii)} the coefficients of each $f_i$ such that the overall polynomial has the best approximation to $\sign(x)$ over the interval $[-1, 1]$. To decompose this problem, we first fix the degrees and then find the best coefficients for our sparse basis in \ref{eq:basis}. Because sign function is non-smooth while polynomials is smooth, there is an inherent conflict near zero: $\text{sign}(\epsilon) = 1$ but $f_i(epsilon) \approx 0$ for small $\epsilon$. Consequently we only consider the interval $[\epsilon, 1]$ \footnote{we consider the positive side because it is odd function.} for approximation.

Following \cite{lee2022tdsc-minimax-approximation-sign}, we applied Remez algorithm to get the optimal polynomial when given the polynomial degrees and $\epsilon$.

\subsection{Remez algorithm}

The Remez algorithm is a well-known method for finding minimax polynomial approximations to a given function over a specified interval. In our case, we apply the Remez algorithm to the composite polynomial structure defined above. 

We aimed to map the interval $[\epsilon, 1]$ to $1$. Denote image of $f_1 \circ f_2 \circ ... \circ f_i$ as $[a_i,b_i]$, where  $a_i = \epsilon$ and $b_i = 1$. The use of Remez algorithm is as follow:

\textit{Given a polynomial space spanned by basis $\{b_i(x)\}_{i=1,...,k}$, the Remez algorithm finds the coefficients such that the polynomial minimizes the maximum absolute value from a target function (in our case, $y = 1$) over the interval $[a, b]$.}


\begin{enumerate}[leftmargin=*,label=\arabic*.]
    \item \textbf{Initialize extremal points.} \\
      We will maintain $k+1$ extremal points
      \(\{x_i\}_{i=1}^{k+1}\subset[a,b]\).  Start by the Chebyshev nodes on \([a,b]\).
    \item \textbf{Main iteration (up to \(\text{maxiter}\) times).}  For \(\text{iter} = 1,\dots,\text{maxiter}\):
      \begin{enumerate}[label=\alph*.]
        \item \textbf{Build and solve the alternation system.}  At the current extremal points \(x_i\), enforce
        \[
          f(x_i)\;-\;\sum_{j=1}^k c_j\,b_j(x_i) \;=\; (-1)^{\,i-1}\,E,
          \quad i=1,\dots,n+1.
        \]
        \item \textbf{Get the root.}  Let $e(x) \;=\; f(x) \;-\;\sum_{j=1}^n c_j\,\varphi_j(x).$ Find all the root and sort them: $a < z_1 < z_2 < \cdots < z_n < b.$
  
        \item \textbf{Find the new set of \(n+1\) extremal points.}  The zeros \(\{z_m\}\) divide \([a,b]\) into \(n+1\) subintervals:
        \[
          [\,z_0=a,\;z_1\,],\quad [\,z_1,z_2\,],\;\dots,\;[\,z_n,\;z_{n+1}=b\,].
        \]
        On each subinterval \([z_{\ell}, z_{\ell+1}]\), locate a point where \(\lvert e(x)\rvert\) is maximized. If does not yield a valid critical point, compare \(\lvert e(x_{\ell})\rvert\) and \(\lvert e(x_{\ell+1})\rvert\) and pick whichever endpoint has larger absolute error.  Collect these \(n+1\) points into \(\{\,x^{\text{new}}_i\}_{i=1}^{n+1}\).
  
      \end{enumerate}
  
    \item \textbf{Check convergence.}  Stop if the changes of $x_i$ is small or reached maximum iteration.
  \end{enumerate}
  The algorithm is given in \red{TBD}.

\subsection{Neural Network Refinement}

Because our initial goal is to approximate the ReLU function, so there is room to improve upon the polynomial obtained via the Remez algorithm. Therefore, we perform a further gradient‐based refinement using the current polynomial as an initial guess. The trainable parameters are its coefficients, denoted \(\{\gamma_{i},\ell_{i},r_{i}\}_{i=1}^{N}\) for \(N\) polynomials. The polynomial is parameterized as:

\begin{align}
    p_{0} \;=\; -\bigl(1 + r\bigr), 
      \quad
      p_{1} \;=\; -\bigl(1 - \ell\bigr), 
      \quad
      p_{2} \;=\; 0, 
      \quad
      p_{3} \;=\; 1 - \ell, 
      \quad
      p_{4} \;=\; 1 + r. \\
      \widetilde{f}(x)
      \;=\; x \;+\; \gamma\,(x - p_{0})(x - p_{1})(x - p_{2})(x - p_{3})(x - p_{4}).
\end{align}

We adopt the re-parameterized polynomial basis in place of the standard monomial or Chebyshev bases because it delivers far greater numerical stability. The parameters \(\ell\) and \(r\) respectively represent the left and right endpoints of the interval $[0,1]$. You can think of this re-parameterization as a kind of residual network (ResNet) that helps stabilize training. In addition, it’s trivial to enforce interval constraints---for example, to ensure that the peak value from one iteration never exceeds the right fixed point of the next.
    
As for loss design, we wish \(\widetilde{f}_1 \circ \widetilde{f}_2 \circ ... \circ \widetilde{f}_n = y_{\mathrm{final}}(x) \approx x\) uniformly on $x\in[0,1.005]$.  
The $l_\infty$ loss is defined as:
\[
l_{\infty} \;=\; \max_{\,x}\bigl|y_{\mathrm{final}}(x) - x\bigr|
\]
with respect to the \(3N\) real parameters \(\{\gamma_{i},\ell_{i},r_{i}\}_{i=1}^{N}\). We use pytorch and Adam optimizer to minimize the loss. The training finished within 100,000 iterations.

\subsection{Empirical formula}

When $K$ is greater than $15$, the Remez algorithm is not numerically stable. Fortunately, we can provide an empirical $f_s(x)$ with analytical form:
\begin{align*}
    f_s(x) = x + \frac{1}{6} \cdot \sum_{k=1}^K \sqrt{2^{k+1} + 1} \cdot \left( 1 + 2^{-(k+1)} \right)^{2^k} \cdot x \cdot (1 - x^2)^{2^k}
\end{align*}
As $k$ goes larger, the coefficients grow roughly as $\frac{\sqrt{e}}{6} \cdot 2^{\frac{k+1}{2}}$. Since in our case, $K$ is less than $40$, the maximum coefficient is still below $10^6$, which is within the safe range of single precision. We can further combine Remez with this analytical form. 

Figure~\ref{fig:comparison} illustrates the approximation error in different methods. 
\input{figs/comparison.tex}

\subsection{GPU Tensor Core implementation}

We implemented the new fixed point iteration in GPU's Tensor Core. For \texttt{Float16}, the speed-up is significant. For a $10,000 \times 10,000$ symmetric matrix, we only need $0.1$s to approximate the PSD cone projection within $10^{-4}$ relative error (20 matrix-matrix multiplications) in H100. In comparison, full eigenvalue decomposition in \texttt{Float32} needs $1$s. 

However, the difficulty lies in Tensor Core's \texttt{Float32}. It only has three-decimal accuracy. If I return to use ``normal'' \texttt{Float32} in CUDA cores, each matrix-matrix multiplication needs around $40$ ms, which is 10 times slower than \texttt{Float16}'s matrix-matrix multiplication in Tensor Core. \blue{Is there a way to utilize several \texttt{Float16}'s matrix-matrix multiplication to mimic ``true'' \texttt{Float32} accuracy?}


==> sections/method.tex <==
%!TEX root = ../main.tex

\section{Composite Polynomial Filter Design}
\label{sec:methods}

\red{
  This section needs major rewriting:
  \begin{itemize}
    \item The section should start with a problem formulation that echos the major design challenge in the introduction, i.e., given a fixed budget of matrix-matrix multiplications, how to construct an optimal composite polynomial filter. This should be clearly formulated as a minimax optimization problem with outer $\min$ over the polynomial components and inner $\max$ over $x \in [-1,1]$.
    \item After the problem statement, we should discuss why it is difficult, if not impossible, to solve the seemingly low-dimensional optimization problem. One potential strategy is to use Lasserre's minimax polynomial optimization hierarchy, but we should comment that this is unlikely going to be tractable.
    \item This difficulty then justisfies our two-stage design strategy. In stage one, we replace the ReLU with the sign function, for which we can use Remes algorithm to find optimal coefficients. In stage two, we perform local gradient-based optimization to finetune the coefficients. 
    \item Lastly, we should comment that, although our framework does not guarantee finding the globally optimal polynomial coefficients, we do offer guarantees on the worst-case approximation error, once the polynomial coefficients are computed. This should be stated as a theorem, and the proof should be very simple.
    \item The Remes algorithm can be presented in Appendix.
    \item Be careful, and consistent about the notation used in the introduction
    \begin{itemize}
      \item $n$: dimension of the PSD cone 
      \item $d$: degree of each polynomial component
      \item $T$: number of components in the composite filter
    \end{itemize}

    \item I would also have a table listing (a) different composite polynomial filter design choices, and (b) their corresponding worst-case approximation errors. These different designs should come from, for example, (1) Newton-Schulz, (2) the one in \cite{francisco17laa-fixedpoint-approximate-psdcone}, (3) the one in \cite{amsel25arxiv-polar-express}, (4) feeding (2) and (3) into our gradient descent, (5) ours.
  \end{itemize}
}

We frame the problem of optimizing the polynomial coefficients as a minimax approximation task. To obtain an initial solution, we apply the Remez algorithm to greedily approximate the sign function, $\sign(x)$. The resulting polynomial then serves as the starting point for a gradient-based refinement step, which further improves the approximation by directly optimizing its coefficients. Once the final polynomial is computed, we certify its worst-case approximation error by comparing it against established benchmarks.

\subsection{Problem formulation}
Given a fixed degree sequence $\{d_t\}_{i=1}^T$, we seek the optimal composite polynomial
\[
f_1 \circ f_2 \circ \cdots \circ f_T
\]
that approximates $\frelu(x)$ on $[-1,1]$ in the minimax sense:

\begin{align}\label{eq:minimax-relu}
    \min_{f_1,f_2,...f_T} \max_{x \in [-1, 1]} ~~~&|f_1 \circ f_2 \circ ... \circ f_T(x) - \frelu(x)| \tag{MINIMAX-RELU}\\
    \subject &f_t \in \mathbb{R}_{\leq d_t}[x]
    \notag
\end{align}

Though it is natural to direct approximate the ReLU function,  it introduces substantial challenges when solving this ostensibly simple optimization problem. One straight forward strategy is approximate the ``max'' operator by dense sampling:

\begin{align}
  \min_{f_1,f_2,...f_T} \max_{j = 1,2,...,N} ~~~&|f_1 \circ f_2 \circ ... \circ f_T(x_j) - \frelu(x_j)| \tag{SAMPLE-RELU}\\
  \subject &f_t \in \mathbb{R}_{\leq d_t}[x]
  \notag\\
  &x_j = -1 + \frac{2j}{N-1}, j = 1,2,...,N \notag
\end{align}

Because of the highly non-linear nature of the ReLU function, the optimization landscape is extremely complex, with many local minima. This makes it difficult to find a good solution without good initial guess, \red{see result in...}. An alternative way to solve \eqref{eq:minimax-relu} is to use \red{Lasserre's ...}

Following \cite{lee22tdsc-minimax-approximation-sign}, the minimax composite polynomial of a sign function can be solved by composite a series of minimax polynomial.
So instead of directly solve \eqref{eq:minimax-relu}, we approximate the sign function and employ the identity $\frelu(x) = 0.5\,x\,(1 + \sign(x))$.

Since \(\sign(x)\) is odd, we may restrict our attention to odd polynomials. Assuming \(d_t = 2p_t + 1\) and the problem is stated:

\begin{align}\label{eq:minimax-sign}
    \min_{f_1,f_2,...f_T} \max_{x \in [-1, 1]} |f_1 \circ f_2 \circ ... \circ f_T(x) - \sign(x)| \tag{MINIMAX-SIGN}\\
    \text{where } f_t = \sum_{j=0}^{p_t} c_{t,j} x^{2j + 1} , c_{t,j} \in \mathbb{R} \notag
    \notag
\end{align}

Because the sign function is non-smooth, whereas polynomial functions are smooth, an inherent conflict arises near zero: $\text{sign}(\epsilon)=1$ but $f_t(\epsilon)\approx0$ for small $\epsilon$. Consequently, we restrict our attention to the interval $[\epsilon,1]$. In our experiments, we set $\epsilon=10^{-3}$.

Following \cite{lee22tdsc-minimax-approximation-sign}, we employ the Remez algorithm to obtain the optimal polynomial for a given polynomial degree $\{d_t\}_{i=1}^T$ and $\epsilon$.

% To maximize the sharpness of a polynomial at the origin, it is desirable to use high-degree polynomials. However, the degree is constrained by the number of multiplications that can be performed within given computational limits. To overcome this bottleneck, we introduce a \textbf{composite polynomial structure} --- a construction that strategically combines multiple lower-degree polynomials. This structure enables us to effectively simulate a high-degree polynomial, achieving increased sharpness at the origin while remaining within a feasible computational budget.
% \subsection{Sparse basis}
% Sparse basis is designed to aggressively lift up the polynomial degrees within the limited number of multiplications. Inspired by Newton-Schulz iteration, we define our new ``basis'' as:
% \begin{align}\label{eq:basis}
%     x, \ \left\{ x \cdot (1 - x^2)^{2^k} \right\}_{k=0}^K \tag{BASIS}
% \end{align}
% To generate this set, we require only $K{+}1$ multiplications. This set can then be directly passed to the Remez algorithm to construct a feasible composite polynomial, as in~\cite{amsel2025arxiv-polar-express,lee2022tdsc-minimax-approximation-sign}. However, care must be taken, as our set of polynomials does not form a true basis for the space of polynomials of degree at most $2^K$. As a result, the Remez algorithm may fail to converge. Nevertheless, if the Remez algorithm does converge, the resulting coefficients are indeed minimax optimal over the given composite structure. In this case, we get our composite polynomial as 
% \begin{align*}
%     f_o(x) = c_{-1} \cdot x + \sum_{k=0}^K c_k \cdot x \cdot (1 - x^2)^{2^k}
% \end{align*}
% where ``o'' represents oscillating: $f_o$'s effect is to provide large slope near $0$. In the end of the composition, we also need some smoothing function to get high-accuracy approximation:
% \begin{align*}
%     f_s(x) = 1.5 x - 0.5 x^3
% \end{align*}
% which is exactly the Newton-Schulz iteration. 

% \subsection{Composite architecture}

% We measure the approximation error in the $l_\infty$ norm using dense sampling. A natural idea is to approximate the ReLU function directly, but this creates difficulties when forming composite functions: because $\frelu(x)$ has a non‐constant image, one cannot use a polynomial with a shrinking image to build the composite formula. Instead, we approximate the sign function and employ the identity: $\frelu(x) = 0.5 x \cdot (1 + \sign(x))$. 

% To determine the composite polynomial $f_1 \circ f_2 \circ ... \circ f_n$, we must calculate \textbf{(i)} the degree (or degree of freedom here) of each $f_i$ and \textbf{(ii)} the coefficients of each $f_i$ such that the overall polynomial has the best approximation to $\sign(x)$ over the interval $[-1, 1]$. To decompose this problem, we first fix the degrees and then find the best coefficients for our sparse basis in \ref{eq:basis}. Because sign function is non-smooth while polynomials is smooth, there is an inherent conflict near zero: $\text{sign}(\epsilon) = 1$ but $f_i(\epsilon) \approx 0$ for small $\epsilon$. Consequently we only consider the interval $[\epsilon, 1]$ \footnote{we consider the positive side because it is odd function.} for approximation.

% Following \cite{lee2022tdsc-minimax-approximation-sign}, we applied Remez algorithm to get the optimal polynomial when given the polynomial degrees and $\epsilon$.

\subsection{Stage 1: Remez algorithm}

The Remez algorithm is a well-known method for finding minimax polynomial approximations to a given function over a specified interval. In our case, we apply the Remez algorithm to the composite polynomial structure defined above. 

We aimed to map the interval $[\epsilon, 1]$ to $1$. Denote image of $f_1 \circ f_2 \circ ... \circ f_t$ as $[l_t, u_t]$, where  $l_1 = \epsilon$ and $u_1 = 1$. The use of Remez algorithm is as follow:

\textit{Given a polynomial space spanned by basis $\{b_i(x)\}_{i=1,...,k}$, the Remez algorithm finds the coefficients such that the polynomial minimizes the maximum absolute value from a target function (in our case, $y = 1$) over the interval $[a, b]$.}


\begin{enumerate}[leftmargin=*,label=\arabic*.]
    \item \textbf{Initialize extremal points.} \\
      We will maintain $k+1$ extremal points
      \(\{x_i\}_{i=1}^{k+1}\subset[a,b]\).  Start by the Chebyshev nodes on \([a,b]\).
    \item \textbf{Main iteration (up to \(\text{maxiter}\) times).}  For \(\text{iter} = 1,\dots,\text{maxiter}\):
      \begin{enumerate}[label=\alph*.]
        \item \textbf{Build and solve the alternation system.}  At the current extremal points \(x_i\), enforce
        \[
          f(x_i)\;-\;\sum_{j=1}^k c_j\,b_j(x_i) \;=\; (-1)^{\,i-1}\,E,
          \quad i=1,\dots,n+1.
        \]
        \item \textbf{Get the root.}  Let $e(x) \;=\; f(x) \;-\;\sum_{j=1}^n c_j\,\varphi_j(x).$ Find all the root and sort them: $a < z_1 < z_2 < \cdots < z_n < b.$
  
        \item \textbf{Find the new set of \(n+1\) extremal points.}  The zeros \(\{z_m\}\) divide \([a,b]\) into \(n+1\) subintervals:
        \[
          [\,z_0=a,\;z_1\,],\quad [\,z_1,z_2\,],\;\dots,\;[\,z_n,\;z_{n+1}=b\,].
        \]
        On each subinterval \([z_{\ell}, z_{\ell+1}]\), locate a point where \(\lvert e(x)\rvert\) is maximized. If does not yield a valid critical point, compare \(\lvert e(x_{\ell})\rvert\) and \(\lvert e(x_{\ell+1})\rvert\) and pick whichever endpoint has larger absolute error.  Collect these \(n+1\) points into \(\{\,x^{\text{new}}_i\}_{i=1}^{n+1}\).
  
      \end{enumerate}
  
    \item \textbf{Check convergence.}  Stop if the changes of $x_i$ is small or reached maximum iteration.
  \end{enumerate}
  The algorithm is given in \red{TBD}.

We can certify the composite polynomial through greedy search is indeed optimal. We state the theorem here:

\begin{theorem}[Overall Optimality]
  Let $d$ be odd and define $\ell_1=\ell$ and $u_1=u$. For $t=1,\dots,T$ define
  \begin{align}
  \label{eq:9a}
  p_t &= \argmin_{p\in P_{d_t}^{\mathrm{odd}}}\,\max_{x\in[\ell_t,u_t]} \bigl|1-p(x)\bigr|,\\
  \label{eq:9b}
  \ell_{t+1} &= \min_{x\in[\ell_t,u_t]} p_t(x),\\
  \label{eq:9c}
  u_{t+1} &= \max_{x\in[\ell_t,u_t]} p_t(x).
  \end{align}
  Then the new error, lower and upper bounds can be computed through
  \begin{equation}\label{eq:10}
  \ell_{t+1} = p_t(\ell_t), 
  \quad
  u_{t+1} = 2 - \ell_{t+1},
  \quad
  \max_{x\in[\ell_t,u_t]} \bigl|1 - p_t(x)\bigr| = 1 - \ell_{t+1}.
  \end{equation}
  Furthermore, the composition
  \[
  p^* := p_T \circ p_{T-1} \circ \cdots \circ p_1
  \]
  is optimal and the error is given by:
  \begin{equation}\label{eq:11}
  \max_{x\in[\ell,u]} \bigl|1 - p^*(x)\bigr|
  =
  \min_{\substack{p = p_T\circ p_{T-1}\circ \cdots \circ p_1\\ p_t\in P_{d_t}^{\mathrm{odd}}}}
  \max_{x\in[\ell,u]} \bigl|1 - p(x)\bigr|
  = 1 - \ell_{T+1}.
  \end{equation}
  \end{theorem}

\textbf{Smooth function}. In practice we often
add other several Newton-Schulz polynomials after the minimax composite function to make the polynomial stable and accurate around $1$.
\red{may explain more here}.

\subsection{Stage 2: Neural Network Refinement}

Because our initial goal is to approximate the ReLU function, so there is room to improve upon the polynomial obtained via the Remez algorithm. Therefore, we perform a further gradient‐based refinement using the current polynomial as an initial guess. We choose $d_t = 5$ in this section and the trainable parameters are its coefficients, denoted \(\{\gamma_{i},\ell_{i},r_{i}\}_{i=1}^{N}\) for \(N\) polynomials. The polynomial is parameterized as:

\begin{align}
    p_{0} \;=\; -\bigl(1 + r\bigr), 
      \quad
      p_{1} \;=\; -\bigl(1 - \ell\bigr), 
      \quad
      p_{2} \;=\; 0, 
      \quad
      p_{3} \;=\; 1 - \ell, 
      \quad
      p_{4} \;=\; 1 + r. \\
      \widetilde{f}(x)
      \;=\; x \;+\; \gamma\,(x - p_{0})(x - p_{1})(x - p_{2})(x - p_{3})(x - p_{4}).
\end{align}

We adopt the re-parameterized polynomial basis in place of the standard monomial or Chebyshev bases because it delivers far greater numerical stability. The parameters \(\ell\) and \(r\) respectively represent the left and right endpoints of the interval $[0,1]$. You can think of this re-parameterization as a kind of residual network (ResNet) that helps stabilize training. In addition, it’s trivial to enforce interval constraints----for example, to ensure that the peak value from one iteration never exceeds the right fixed point of the next.
    
As for loss design, we wish \(\widetilde{f}_1 \circ \widetilde{f}_2 \circ ... \circ \widetilde{f}_n = y_{\mathrm{final}}(x) \approx x\) uniformly on $x\in[0,1.005]$.  
The $l_\infty$ loss is defined as:
\[
l_{\infty} \;=\; \max_{\,x}\bigl|y_{\mathrm{final}}(x) - x\bigr|
\]
with respect to the \(3N\) real parameters \(\{\gamma_{i},\ell_{i},r_{i}\}_{i=1}^{N}\). We use pytorch and Adam optimizer to minimize the loss. The training finished within 100,000 iterations.

